Domain Adaptive Imitation Learning

We study the question of how to imitate tasks across domains with discrepancies such as embodiment, viewpoint, and dynamics mismatch. Many prior works require paired, aligned demonstrations and an additional RL step that requires environment interactions. However, paired, aligned demonstrations are seldom obtainable and RL procedures are expensive. We formalize the Domain Adaptive Imitation Learning (DAIL) problem, which is a unified framework for imitation learning in the presence of viewpoint, embodiment, and dynamics mismatch. Informally, DAIL is the process of learning how to perform a task optimally, given demonstrations of the task in a distinct domain. We propose a two step approach to DAIL: alignment followed by adaptation. In the alignment step we execute a novel unsupervised MDP alignment algorithm, Generative Adversarial MDP Alignment (GAMA), to learn state and action correspondences from \emph{unpaired, unaligned} demonstrations. In the adaptation step we leverage the correspondences to zero-shot imitate tasks across domains. To describe when DAIL is feasible via alignment and adaptation, we introduce a theory of MDP alignability. We experimentally evaluate GAMA against baselines in embodiment, viewpoint, and dynamics mismatch scenarios where aligned demonstrations don't exist and show the effectiveness of our approach.

==> format_old/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> proofs/compatible_rl_js.tex <==
\begin{lemma}
If $\gM_x \sim \gM_y$ and $\gM^*_x$ and $\gM^*_y$ are maximal reductions to $\gM_x$ and $\gM_y$ respectively, then there exists an isomorphism between $\gM^*_x$ and $\gM^*_y$.
\end{lemma}
\begin{proof}
Since $\gM_x \sim \gM_y$, there exists $\gM^*$ such that $\gM^* \leq \gM_x$ and $\gM^* \leq \gM_y$. Therefore, there exists a maximal reduction of $\gM_x$ or $\gM_y$ that is also a reduction of $\gM^*$. The uniqueness of a maximal reduction ensures that the maximal reduction of $\gM_x$ or $\gM_y$ must be a reduction of $\gM^*$.
\end{proof}

\begin{theorem}
If $\mx \sim \my$, then if for some $f^*$ and $g^*$ such that:
$$
\pi_{x} = g \circ \pi_{y} \circ f \text{ is optimal in } \gM \quad \text{and} \quad \rho_{\pi_{x}}(\tau_{y}) = \rho_{\pi_{y}}(\tau_{y})
$$ 
then there exists $\gM^*$ such that $\gM^*$ is a maximal reduction of $\mx$ and $\my$, 
$\gM^* \leq_{\phi_x, \psi_x} \gM_x$ and $\gM^* \leq_{\phi_y, \psi_y} \gM_y$, where $f^* \in \phi_y^{-1} \circ \phi_x$ and $g^* \in \psi_x^{-1} \circ \psi_y$.
\end{theorem}
\begin{proof}
Consider the mapping from $(\gS^\star, \gA^\star)$ defined as $h^* = (\phi_y \circ f^* \circ \phi_x^{-1}, \psi_{y}^{-1} \circ g^* \circ \psi_x)$, we show this forms a valid homomorphism from $\gM^*$ to $\gM^*$.

\paragraph{Dynamics preservation} 
For all $s^* \in \gS^*$ if $a^*$ is an optimal action for $s^*$ then 

\js{todo}
As $\rho_{\pi_{x}}(\tau_{y}) = \rho_{\pi_{y}}(\tau_{y})$, $f$ has to be a surjection.

\paragraph{Reward preservation} \js{todo}

Since $\gM^*$ is a maximal reduction, there does not exist non-identity automorphisms, so $(\phi_y \circ f^* \circ \phi_x^{-1}, \psi_{y}^{-1} \circ g^* \circ \psi_x)$ defines an identity relationship:
\begin{align*}
    \phi_y \circ f^* \circ \phi_x^{-1} = I \\
    \psi_{y}^{-1} \circ g^* \circ \psi_x = I
\end{align*}

\end{proof}

==> proofs/reduction_uniqueness.tex <==
\begin{lemma} The maximal reduction $\mc{M}^*$ of an MDP $\mc{M}$ is ``unique'', i.e. all the maximal reductions are isomorphic to each other. 
\label{lemma:max_reduction}
\end{lemma}
\begin{proof}
If the maximal reduction is not unique, then $\exists \gM_1, \gM_2$ such that $\gM_1$ and $\gM_2$ are both maximal reductions of $\gM$ and that $\gM_1$ and $\gM_2$ are not equivalent. We proceed to show that we can construct a $\phi_3$ and $\psi_3$ such that the corresponding reduction is a strictly smaller reduction of $\gM_1$ and $\gM_2$, which proves the lemma by contradiction.

(Construction of $\phi_3$) For $s, s' \in \mc{S}$, we define $s$ is ``reachable'' to $s'$ if there exists a sequence $s_1, s_2, \ldots, s_{k-1}$ such that $\forall i=0, \ldots, k$, 
\begin{align}
\phi_1(s_i) = \phi_1(s_{i+1}) \quad \text{or} \quad \phi_2(s_i) = \phi_2(s_{i+1}) \quad \text{holds.} \label{eq:state12}
\end{align}
where $s_0 := s, s_{k} := s'$
The ``reachable'' relationship defines an equivalence class $[\gS_i]$ and we simply assign $\phi_3(s) = i$ if $s \in \gS_i$. 

(Verifying dynamics preservation for $\phi_3$) For all $s, s' \in \mS$ such that $\phi_3(s) = \phi_3(s')$ and corresponding $s_1, s_2, \ldots, s_{k-1}$ sequence, we have $\forall a \in \gA, i \in 0, \ldots, k$:
$$
\phi_1(T(s_{i}, a)) = \phi_1(T(s_{i+1}, a)) \quad \text{or} \quad \phi_2(T(s_{i}, a)) = \phi_2(T(s_{i+1}, a)),
$$
from the definition of dynamics preservation and Equation~\ref{eq:state12}.
Therefore $\phi_3(T(s_{i}, a)) = \phi_3(T(s_{i+1}, a))$, and so $\phi_3(T(s, a)) = \phi_3(T(s', a))$ due to transitive property of equality. 

(Construction of $\psi_3$) We repeat a similar argument for actions. We define $a$ is ``reachable'' to $a'$ if there  exists a sequence $a_1, a_2, \ldots, a_{k-1}$ such that $\forall i=0, \ldots, k$, 
\begin{align}
    \psi_1(a_i) = \psi_1(a_{i+1}) \quad \text{or} \quad \psi_2(a_i) = \psi_2(a_{i+1}) \quad \text{holds.} \label{eq:action12}
\end{align}
Again, this defines an equivalence class $[\gA_i]$ and we assign $\psi_3(a) = i$ if $a \in \gA_i$. 

(Verifying dynamics preservation for $\psi_3$) For all $a, a' \in \gA$ such that $\phi_3(a) = \phi_3(a')$ and corresponding $a_1, a_2, \ldots, a_{k-1}$ sequence, we have $\forall s \in \gS, i \in 0, \ldots, k$:
$$
\phi_1(T(s, a_{i})) = \phi_1(T(s, a_{i+1})) \quad \text{or} \quad \phi_2(T(s, a_{i})) = \phi_2(T(s, a_{i+1})),
$$
which is from the definition of dynamics preservation and Equation~\ref{eq:action12}.
Thus $\phi_3(T(s, a_{i})) = \phi_3(T(s, a_{i+1}))$ and so $\phi_3(T(s, a)) = \phi_1(T(s, a'))$ holds due to transitive property of equality. 

Moreover, for $s, s' \in \gS, a, a' \in \gA$ such that $\phi_3(s) = \phi_3(s')$ and $\psi_3(a) = \psi_3(a')$ \js{we preserve the optimal policy, will flush this out once we settle with a formalization.}

% Since $\gM_1$ and $\gM_2$ are not equivalent, so there exists some state or action where Equation~\ref{eq:state12} or~\ref{eq:action12} holds true. 
Hence $\gM_3 \leq \gM_1$ and $\gM_3 \neq \gM_1$, and this contradicts the assumption that $\gM_1$ is a minimal reduction; the same argument holds for $\gM_2$.
\end{proof}

==> sections/dump.tex <==
% \input{proofs/reduction_uniqueness.tex}

% \begin{corollary}
% If there exists $\mc{M}$ such that $\mc{M} \leq \mx$ and $\mc{M} \leq \my$, then $\mx \sim \my$.
% \label{corollary:exist_reduction}
% \end{corollary}

% \begin{lemma} Let $\pi_{\mc{\bar{M}}}^*$ be optimal in $\bar{\mc{M}} \leq \mc{M}$. Then $\pi_{\mc{M}}(a | s) = \frac{\pi_{\mc{\bar{M}}}^*(\psi(a) | \phi(s))}{|\phi^{-1}(a)|}$ is optimal in $\mc{M}$.
% \label{lemma:pi_transfer}
% \end{lemma}
% \begin{comment}
% Conversely, let $\pi_{\mc{M}}^*$ be an optimal policy in $\mc{M}$. Then, $\pi_{\mc{\bar{M}}}(\bar{a} | \bar{s}) = \pi_{\mc{M}}^*(s | a)$ for any $s \in \phi^{-1}(\bar{s}), a \in \phi^{-1}(\bar{a})$ is optimal. 
% \end{comment}


% Lemma \ref{corollary:exist_reduction} implies that if two MDPs have a common reduction, then they also have equivalent maximal reductions.

% \begin{theorem}
% If $\mx \geq_{\phi, \psi} \my$, then $p_{\pi_{x}}(\tau_{y}) = p_{\pi_{y}}(\tau_{y})$ and $\pi_{x} = g \circ \pi_{y} \circ f$ is optimal if and only if $f = \phi$ and $g(a^{y}) \in \psi^{-1}(a^{y}) ~ \forall a^{y} \in \ay$. 
% \end{theorem}

% \begin{proof}
% $\leftarrow$
% We define $f$ and it's inverse as $f = \phi, f^{-1}(y) \in \phi^{-1}(y)$ and $g(a^{y}) \in \psi^{-1}(a^{y})~ \forall a^{y} \in \ay$. 
% \begin{align*}
% p_{\pi_{x}}(\tau_{y}) &= \sum_{\mathclap{s^{x}_{0} \in \phi^{-1}(s^{y}_{0})}} \eta_{x}(s^{x}_{0})\pi_{y}(a^{y}_{0} | s^{y}_{0}) \sum_{\mathclap{s^{x}_{1} \in \phi^{-1}(s^{y}_{1})}} \px(s^{x}_{1} | s^{x}_{0}, g(a^{y}_{0})) \pi_{y}(a^{y}_{1} | s^{y}_{1}) \sum_{\mathclap{s^{x}_{2} \in \phi^{-1}(s^{y}_{2})}} \px(s^{x}_{2} | s^{x}_{1}, g(a^{y}_{1})) \pi_{y}(a^{y}_{2} | s^{y}_{2})\cdots \\
% &= \sum_{\mathclap{s^{x}_{0} \in \phi^{-1}(s^{y}_{0})}} \eta_{x}(s^{x}_{0}) \Big(\pi_{y}(a^{y}_{0} | s^{y}_{0}) \sum_{\mathclap{s^{x}_{1} \in \phi^{-1}(s^{y}_{1})}} \px(s^{x}_{1} | f^{-1}(s^{y}_{0}), g(a^{y}_{0})) \Big)
% \Big(\pi_{y}(a^{y}_{1} | s^{y}_{1})\sum_{\mathclap{s^{x}_{2} \in \phi^{-1}(s^{y}_{2})}} \px(s^{x}_{2} | f^{-1}(s^{y}_{1}), g(a^{y}_{1})) \Big) \cdots 
% \\
% &= \sum_{\mathclap{s^{x}_{0} \in \phi^{-1}(s^{y}_{0})}} \eta_{x}(s^{x}_{0}) \prod_{t = 0}^{T-1} \Big( \pi_{y}(a^{y}_{t} | s^{y}_{t}) \sum_{\mathclap{s^{x}_{t+1} \in \phi^{-1}(s^{y}_{t+1})}} \px(s^{x}_{t+1} | f^{-1}(s^{y}_{t}), g(a^{y}_{t})) \Big) 
% \\
% &= \eta_{y}(s^{y}_{0}) \prod_{t = 0}^{T-1} \pi_{y}(a^{y}_{t} | s^{y}_{t}) \py(s^{y}_{t+1} | s^{y}_{t}, a^{y}_{t})
% \end{align*}
% The second step holds since $\px(s^{x}_{i+1} | s^{x}_{i}, a^{x}_{i}) = \px(s^{x}_{i+1} | s^{x}_{i}', a^{x}_{i})$ for $\phi(s^{x}_{i}) =  \phi(s^{x}_{i}')$ and the last step holds since $(\phi, \psi)$ is a homomorphism. Optimality of $\pi_{x}$ directly follows from Lemma \ref{lemma:pi_transfer}. 

% \rightarrow 


% \end{proof}

% \begin{comment}
% \begin{align*}
% \rho_{\pi_{y}^*}^{y}(s^{y}, a^{y}, s^{y}') &= \sum_{t = 0}^{T - 1} \rho_{\pi_{y}^*}^{y}(s_{t}^{y} = s^{y}, a_{t}^{y} = a^{y}, s_{t+1}^{y} = s^{y}')\\
% &=  \sum_{t = 0}^{T - 1} \sum_{\substack{s^{x} \in \phi^{-1}(s^{y}),\\
%                               a^{x} \in \psi^{-1}(a^{y}) \\
%                               s^{x}' \in \phi^{-1}(s^{y}')}}
% \rho_{\pi_{y}^*}^{y}(s_{t}^{y} = s^{y}, a_{t}^{y} = a^{y}, s_{t+1}^{y} = s^{y}')
% \end{align*}
% \end{comment}


% \input{proofs/compatible_rl_js.tex}




% For brevity, we will occasionally omit $\phi, \psi$ and write $\bar{\mc{M}} \leq \mc{M}, \bar{\mc{M}} \simeq \mc{M}$ to denote that there exists some homomorphism/isomorphism from $\mc{M}$ to $\bar{\mc{M}}$. 

% \begin{definition} A reduction $\mc{M}^*$ of $\mc{M}$ is a \textbf{maximal reduction} if and only if $\mc{M}^* \leq \bar{\mc{M}}, ~ \forall \bar{\mc{M}} \leq \gM$, i.e. $\gM^*$ is a reduction of all the MDPs that are reductions of $\gM$.
% \end{definition}

% We now define a MDP pruning operator which reduces the state action space only to states within support of a policy $\pi$. 

% \begin{definition} Let $\Omega$ be the set of all MDPs and $\pi$ a policy in $\mc{M}$. The pruning operation $C_{\pi}: \Omega \rightarrow \Omega$ is a map from $\mc{M} = (\S, \A, P, R, \eta, T)$ to $\tilde{\mc{M}} = (\tilde{\S}, \tilde{\A}, \tilde{P}, \tilde{R}, \tilde{\eta}, \tilde{T})$ such that $\tilde{\S} = supp(\rho_{\pi}(s, a)) | \S, \tilde{\gA} = supp(\rho_{\pi}(s, a)) | \gA, \tilde{P} = P, \tilde{\eta} = \eta, \tilde{R} = R$. 
% \end{definition}
% \js{is this $\vert$ common notation? maybe safer to write using set definition?}



% \begin{lemma}
% Assume that two MDPs $\gM$, $\bar{\gM}$ satisfy $\bar{\gM} \leq_{\phi, \psi} \gM$. 
% Let $\pi_y$ be an optimal policy in $\bar{\gM}$. $\forall s \in \gS, a \in \gA$, if $\phi(s)$ $\psi(a) \in \mathrm{supp}(\pi_y(\cdot | \phi(s)))$, then $a$ is an optimal action under $s$ in $\gM$. % \js{example for uniform policy} \js{support pi(a) in psi-1 (a)}
% \end{lemma}
% \begin{proof}
% Since $\psi(a) \in \mathrm{supp}(\pi_y(\cdot | \phi(s)))$, $\psi(a)$ is an optimal action for state $\phi(s)$ in $\bar{\gM}$, $\bar{O}(\phi(s), \psi(a)) = 1$. \s{how do you know $\phi(s)$ can be reached?}
% Using the optimal policy preservation condition in Definition 1, $O(s, a) = 1$, so $a$ is an optimal action for $s$ in $\gM$.
% \end{proof}

% \begin{corollary}
% Assume that two MDPs $\gM$, $\bar{\gM}$ satisfy $\bar{\gM} \leq_{\phi, \psi} \gM$, and $\pi_y$ is a policy in $\bar{\gM}$. Let $\pi$ denote the policy which first maps a state $s \in \gS$ to $\phi(s)$, obtain an action $a_y \in \bar{\gA}$ with $\pi_y$, and then selects an action from the set $\psi^{-1}(a_y)$. If $\pi_y$ is optimal in $\bar{\gM}$, then $\pi$ is optimal in $\gM$. 
% \end{corollary}
% \s{add the proof. again, the only thing to worry about here is the ``can be visited part'', which is not entirley clear}

% \begin{definition}
% For some policy $\pi$ in an MDP $\gM$ with transition dynamics $P$, 
% we define its \textbf{stationary distribution} as $\rho_{\pi}^{P}(s, a, s') = \sum_{t=0}^{\infty} \gamma^t \mathrm{Pr}(s_t = s, a_t = a, s_{t+1} = s' | \pi, P)$, which is the unnormalized state-action-state triplet distributions that the agent encounters while navigating with policy $\pi$ and transition dynamics $P$.
% \end{definition}


% \begin{definition}
% For some policy $\pi$ in an MDP $\gM$ with transition dynamics $P$, we define its \textbf{triplet occupancy measure} as $\rho_{\pi}^{P}(s, a, s') = \frac{1}{1 - \gamma} \sum_{t=0}^{\infty} \gamma^t \mathrm{Pr}(s_t = s, a_t = a, s_{t+1} = s' | \pi, P)$, which is the unnormalized state-action-state triplet distributions that the agent encounters while navigating with policy $\pi$ and transition dynamics $P$.
% \end{definition}

% \begin{lemma}
% For any policy $\pi$, state space $\gS$ and action space $\gA$, if there exists two valid transition dynamics $P$ and $P'$ such that $P \neq P'$ for some $(s, a, s') \in \mathrm{supp}(\rho_{\pi}^{P}(s, a, s'))$ then 
% $$
% \rho_{\pi}^{P}(s, a, s') \neq \rho_{\pi}^{P'}(s, a, s')
% $$
% for all $s \in \gS, a \in \gA, s' \in \gS$.
% \end{lemma}

% \begin{proof}
% To show that changing the environment dynamics changes the occupancy measure when the policy is fixed, we can consider the following augmented MDP $\gM_a$ with state space $\gS \times \gA$ and action space $\gS$. Under $\gM_a$, we can treat the transition $P$ and $P'$ as valid policies, and treat the policy $\pi$ as defining the transition dynamics $((s_t, a_t), s_{t+1}) \mapsto (s_{t+1}, \pi(a_{t+1} | s_{t+1}))$.

% According to \js{syed} (Theorem 2), occupancy measure and policies has a one-to-one correspondence, so if $P \neq P'$, the corresponding occupancy measure under $\gM_a$ will not be equivalent, i.e., there exists some $((s_t, a_t), s_{t+1})$ such that $\rho_{\pi}^{P}(s_t, a_t, s_{t+1}) \neq \rho_{\pi}^{P'}(s_t, a_t, s_{t+1})$.
% \end{proof}


\begin{theorem}
\label{thm:main}
Two MDPs $\gM_x$ and $\gM_y$ satisfy $\gM_y \leq \gM_x$ and $\text{supp}(\eta_x) = \gS_x$. 
$\pi_y$ is an optimal policy over $\gM_y$ such that $\forall s_y \in \gS_y, a_y \in \gA_y$, $O_y(s_y, a_y) = 1 \iff a_y \in \mathrm{supp}(\pi_y(\cdot | s_y))$. 
Let $f: \gS_x \to \gS_y$ and $g: \gA_y \to \gA_x$ be two deterministic mappings, and $\pi_x = g \circ \pi_y \circ f$. 
Specifically, $\pi_x$ selects an action $a_x$ given a certain state $s_x \in \gS_x$ by mapping it to $f(s_x)$, selecting an action $a_y \in \gA_y$ by sampling from $\pi_y(\cdot|f(s_x))$ and then obtaining its action $a_x = g(a_y)$. 
Let $g^{-1}$ be any function that satisfies $g^{-1} \circ g(a_y) = a_y$ for all $a_y \in \gA_y$, 
Then $(f, g^{-1}) \in \Gamma(\gM_x, \gM_y)$ if and only if $\pi_x \text{ is optimal in } \gM_x \text{ and } \rho_{\pi_y}^{P_y} = \hat{\rho}_{\hat{\pi}_x}^{P_x}$. 
\end{theorem}




\begin{proof}
We define shorthand notations $O_x \triangleq O_{\mx}$ and $O_y \triangleq O_{\my}$, and use $\gQ$ to denote the sampling process with transition kernel defined over $\pi_y$ and $P_y$. We define some state $s_x \in \gS_x$ is ``visited'' by some process $\gP$ if:
\begin{align}
    \sum_{t=0}^{t=\infty} \Pr(s_x^{t} = s_x; \gP) > 0
\end{align}
i.e. there is a non-zero probability that for some time $t$ the random variable $s_x^{t}$ will take value $s_x$. We similarly define this ``visited'' notion for $s_y \in \gS_y$, $a_x \in \gA_x$, $a_y \in \gA_y$.

The theorem is concerned with 4 statements:
\begin{itemize}
    \item $A$: $f, g^{-1}$ preserves optimal policy (Equation \ref{eq:reward})
    \item $B$: $f, g^{-1}$ preserves the transition dynamics (Equation \ref{eq:transition})
    \item $C$: $\pi_x = g \circ \pi_y \circ f \in \Pi^*_{\mx}$
    \item $D$: $\rho_{\pi_y}^{P_y} = \hat{\rho}_{\hat{\pi}_x}^{P_x}$.
\end{itemize}
We proceed to show $A \land B \iff C \land D$. 

($A \land B \Rightarrow C \land D$) Since $\rho_{\pi_y}^{P_y}$ is generated by following the optimal policy $\pi_y$ under $P_y$, 
$$
O_y(s_y, a_y) = 1, \quad \forall (s_y, a_y, s'_y) \in \mathrm{supp}(\rho_{\pi_y}^{P_y}). 
$$ 
We now consider the trajectory sampled with $\pi_x$, which is $\gP(\pi_y, P_x, f, g)$ as in Equation~\ref{eq:policy}. 

% We wish to show by induction that at any time $t$, the distributions of $s^{(t)}_y$ generated by sampling $\gP$ and $\rho_{\pi_y}^{P_y}$ are the same, i.e.
% \begin{align}
% \Pr({s}_y^{(t)} = {s}_y; \gP) = \Pr({s}_y^{(t)} = {s}_y; \pi_y, P_y)
% \end{align}

% If this is true, then by executing $\pi_y$, the corresponding action $a^{(t)}_y$ satisfies $O_y(f(s^{(t)}_x), a^{(t)}_y) = 1$ (by assumption over $\pi_y$). According to optimal policy preservation ($A$),
% $$
% O_y(f(s^{(t)}_x), a^{(t)}_y) = 1, \quad \Rightarrow \quad O_x(s^{(t)}_x, g(a^{(t)}_y)) = 1
% $$ so $\pi_x$ will execute an optimal policy for all time $t$ ($C$).

% \paragraph{Base case: ($t = 0$)} 
% First, according to dynamics preservation ($B$) for the initial state distribution, $s^{(0)}_y \in \eta_y(s^{(0)}_y)$ and $s^{(0)}_y = f(s^{(0)}_x), s^{(0)}_x \sim \eta_x(s^{(0)}_x)$ are the same sampling procedure over $s^{(0)}_y$.

% Then we proceed to show that if $f(s^{(t)}_x)$ can be visited by both $\gP$ and $\rho_{\pi_y}^{P_y}$ at time $t$, then $\pi_x$ will execute an optimal policy at $s^{(t)}_x$, and the next state distribution at time $(t+1)$ visited from $f(s^{(t)}_x)$ are also equivalent. This allows us to use an induction argument, as this is true for $t = 0$, which we just verified for the initial state distributions.
% \paragraph{Inductive step at time $t$} 
Assume that at time $t$ some state $s_y \in \gS_y$ is visited by both $\gP$ and $\gQ$. Both sampling procedures select an $a_y \in \gA_y$ by sampling from $\pi_y(\cdot | s_y)$. $\gQ$ directly produces the next state distribution by $P_y(s_y, a_y)$; $\gP$ indirectly produces the next state distribution by $f(P_x(s_x, g(a_y)))$ where $s_x \in \gS_x, f(s_x) = s_y$. By dynamics preservation ($B$):
$$
P_y(s_y, a_y) = f(P_x(s_x, g(a_y)))
$$
The process in $\gQ$ defines a Markov chain over $\gM_y$, as $(s_y^{(T+1)}, a_y^{(T+1)})$ is independent to $\{(s_y^{(t)}, a_y^{(t)})\}_{t=0}^{T-1}$ conditioned on $(s_y^{(T)}, a_y^{(T)})$, using the transition kernel:
$$
 (s_y, a_y) \mapsto (P_y(s_y, a_y), \pi_y(a_y | P_y(s_y, a_y)))
$$

The process in $\gP$ defines a similar Markov chain as $(s_y^{(T+1)}, a_y^{(T+1)})$ is independent to $\{(s_y^{(t)}, a_y^{(t)})\}_{t=0}^{T-1}$, $\{(s_x^{(t)}, a_x^{(t)})\}_{t=0}^{T-1}$ and $s_x^{T}$ conditioned on $(s_y^{(T)}, a_y^{(T)})$, using the transition kernel:
$$
(s_y, a_y) \mapsto (f(P_x(s_x, g(a_y))), \pi_y(a_y | f(P_x(s_x, g(a_y)))))
$$
where the independence from $s_x^{T}$ is because of ($B$). The transition kernels of $\gP$ and $\gQ$ are equivalent.

% So for all $s_y^{(t)}$ that can be visited and for all $a^{(t)}_y$ that are selected from $\pi_y$ we will get the same distributions for the next state $s^{(t+1)}_y$; the transition of $\gP$ in $\gM_y$ forms a Markov chain.

Therefore, we have:
\begin{align}
    & \hat{\rho}_{\hat{\pi}_x}^{P_x}({s}, {a}, {s}') &\\
    & = \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T-1} \Pr({s}_y^{(t)} = {s}_y, {a}_y^{(t)} = {a}_y, {s}_y^{(t+1)} = {s}'_y; \gP) & \text{(definition)} \\
    & = \lim_{t \to \infty} \Pr({s}_y^{(t)} = {s}_y, {a}_y^{(t)} = {a}_y, {s}_y^{(t+1)} = {s}'_y; \gP) & \text{(Lemma 1)} \label{eq:use-lemma-1} \\
    & = \lim_{t \to \infty} \Pr({s}_y^{(t)} = {s}_y, {a}_y^{(t)} = {a}_y, {s}_y^{(t+1)} = {s}'_y; \pi_y, P_y) & \text{(equivalent transition)}\label{eq:stationary} \\
    % & = \lim_{t \to \infty} \Pr({s}_y^{(t)} = {s}_y; \gP) \pi_y(a_y | s_y) \bb{I}(s'_y = P_y(f(s^{(t)}_x), a^{(t)}_y)) \label{eq:use-transition} \\
    % & = \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T-1} \Pr({s}_y^{(t)} = {s}_y; \pi_y, P_y) \pi_y(a_y | s_y) \bb{I}(s'_y = P_y(f(s^{(t)}_x), a^{(t)}_y)) \label{eq:use-induction} \\
    % & = \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T-1} \Pr({s}_y^{(t)} = {s}_y, {a}_y^{(t)} = {a}_y, {s}_y^{(t+1)} = {s}'_y; \pi_y, P_y) \\
    & = \rho_{\pi_y}^{P_y} &
\end{align}
% where we use Lemma 1 in Equation~\ref{eq:use-lemma-1}.

% \begin{itemize}
%     \item Suppose we start from some $f(s^{(t)}_x)$ that can be visited from which an action $a^{(t)}_y$ is selected by sampling from $\pi_y$. Then the next state distribution on $\gM_y$ is $P_y(f(s^{(t)}_x), a^{(t)}_y)$ and the next state distribution with $\gP$ is $f(P_x(s^{(t)}_x, g(a^{(t)}_y)))$. By dynamics preservation ($B$):
%     $$
%     P_y(f(s^{(t)}_x), a^{(t)}_y) = f(P_x(s^{(t)}_x, g(a^{(t)}_y)))
%     $$
%     So any state $f(s_x^{(t+1)})$ that can be visited by $\rho_{\pi_y}^{P_y}$ is also visited by $\gP$, and the transition dynamics from time $t$ to $(t+1)$ in $\gM_y$ are equivalent. Thus, we denote the transition dynamics in $\gM_y$ induced by $\gP$ as $\hat{P}_y$, and $\hat{P}_y(f(s^{(t)}_x), a_y) = P_y(f(s^{(t)}_x), a_y)$ for all $f(s^{(t)}_x)$ that can be visited and all $a_y$ sampled from $\pi_y(\cdot | f(s^{(t)}_x))$.
% \end{itemize}

% Therefore, $\rho_{\pi_y}^{\hat{P}_y} = \rho_{\pi_y}^{P_y}$ by induction, and $\pi_x$ is optimal at any time $t$ ($C$)




% The trajectory sampled with $\pi_x$ is $\gP(\pi_y, P_x, f, g)$ (Eq.~\ref{eq:policy}), the corresponding state and action in $\gM_x$ satisfy $s_y = f(s_x)$, $g^{-1}(a_x) = a_y$ (since $g^{-1} \circ g = I$). Because $(f, g^{-1})$ preserves optimal policy ($A$), then $O_x(s_x, a_x) = 1$ for all $s_x, a_x$ in the trajectory visited via $\pi_x$. Therefore, $\pi_x$ is an optimal policy in $\gM_x$ ($C$). 

% ($A \land B \land C \Rightarrow D$)
% According to dynamics preservation ($B$), the transition $s'_y = P_y(s_y, a_y) = f(P_x(f^{-1}(s_y), g(a_y)))$ if $(s_y, a_y, s'_y) \in \rho_{\pi_y}^{P_y}$, therefore $P_y$ is equal to the transition dynamics of $\gM_y$ sampling with $\gP$ in Equation~\ref{eq:policy}. The limiting distribution $\bar{\rho}_{\pi_y}^{P_x, f, g}$ is equal to the stationary distribution induced by $\gP(\pi_y, P, f, g)$, which is equal to $\rho_{\pi_y}^{P_y}$.

% As $\pi_x = g \circ \pi_y \circ f$, both $\rho_{\pi_x}^{P_y^{f, g^{-1}}}$ and $\bar{\rho}_{\pi}^{P, f, g}$ are the marginal distributions under the stationary distribution with the same kernel:
% $$
% (s_x, g(a_y), s'_x, f(s_x), a_y, f(s'_x)) \mapsto (s'_x, g(a'_x), s''_x, s'_y, a'_y, f(s''_x))
% $$
% where $a'_y \sim \pi_y(a'_y | s'_y)$ and $s''_x = P_x(s'_x, a_x)$. Therefore, $\rho_{\pi_y}^{P_y} = \rho_{\pi_x}^{P_y^{f, g^{-1}}} = \bar{\rho}_{\pi_x}^{P_x, f, g^{-1}}$.

($C \land D \Rightarrow A$)  %, is sampled from $\bar{\rho}_{\pi_y}^{P_x, f, g}$. 
% satisfy $g^{-1}(a_x) \in \mathrm{supp}(\pi_y(\cdot | f(s_x)))$ and $(f(s_x), g^{-1}(a_x)) \in \mathrm{supp}(\rho_{\pi_y}^{P_y})$ (because $\rho_{\pi_y}^{P_y} = \bar{\rho}_{\pi_y}^{P_x, f, g}$ according to $D$). 
% Because $\pi_x$ policy is optimal, so $O_x(s_x, a_x) = 1$ and thus $g^{-1}(a_x) \in \mathrm{supp}(\pi_y(\cdot | s_y))  \Rightarrow O_x(s_x, a_x) = 1$.
According to the assumptions over $\pi_y$: 
$$O_y(s_y, a_y) = 1 \Rightarrow  (s_y, a_y) \text{ visited by } \gQ, \quad \forall s_y \in \gS_y, a_y \in \gA_y
$$
Because $\rho_{\pi_y}^{P_y} = \hat{\rho}_{\hat{\pi}_x}^{P_x}$ (which is the statement of ($D$)), we have 
$$
(s_y, a_y) \text{ visited by } \gQ \Rightarrow (s_y, a_y) \text{ visited by } \gP, \quad \forall s_y \in \gS_y, a_y \in \gA_y
$$
% \begin{gather}
%   \Rightarrow g^{-1}(a_x) \in \mathrm{supp}(\pi_y(\cdot | f(s_x))), \quad \forall s_x \in \gS_x, a_x \in \gA_x.
% \end{gather} %\Rightarrow O_x(s_x, a_x) = 1$
% ($A$).
For any state $s_x \in \gS_x$ visited with $\gP$ and action $a_x \in \gA_x$ sampled from $\pi_x(\cdot | s_x)$, the corresponding state-action pair in $\gM_y$ visited by $\gP$ is denoted as $(f(s_x), g^{-1}(a_x))$. If $(s_x, a_x)$ is not visited by $\gP$, then $O_y(f(s_x), g^{-1}(a_x)) = 0$.
Since $\pi_x$ is a optimal policy under $\gM_x$ (the statement of ($C$)), we have $O_x(s_x, a_x) = 1$ for $s_x, a_x$ visited by $\gP$. Therefore,
\begin{gather}
 O_y(f(s_x), g^{-1}(a_x)) = 1 \Rightarrow (f(s_x), g^{-1}(a_x)) \text{ visited by } \gP \Rightarrow O_x(s_x, a_x) = 1
\end{gather}
for all $s_x \in \gS_x, a_x \in \gA_x$, which is statement ($A$).

% This verifies the optimal policy preservation property.

($A \land C \land D \Rightarrow B$) 
First we note that 
\begin{align*}
   &  A \land C \land D \to B
   =  \lnot (A \land C \land D) \lor B
   =  \lnot A \lor \lnot C \lor \lnot D \lor B \\
   = \ & (B \lor \lnot A \lor \lnot C) \lor \lnot D 
   = \lnot (\lnot B \land A \land C) \lor \lnot D 
   = \lnot B \land A \land C \to \lnot D
\end{align*}

Therefore, we only need to prove $\lnot B \land (A \land C) \Rightarrow \lnot D$. 
Assume that the dynamics preservation condition is false ($\lnot B$), 
then %either the initial state distribution does not match (and this immediately violates ($D$)),
% \s{why?}
there exists $s_y \in \gS_y$, $a_y \in \gA_y$, $s_x, s'_x \in \gS_x$ and $a_x \in \gA_x$ such that $O_y(s_y, a_y) = 1$, $f(s_x) = f(s_x')$, $a_x = g(a_y)$, yet $$f(P_x(s_x, a_x)) \neq f(P_x(s_x', a_x)).$$ 
Assume that the latter is true.
According to optimal policy preservation ($A$), we have 
$$
O_y(s_y, a_y) = 1 \Rightarrow O_x(s_x, a_x) = 1, O_x(s'_x, a_x) = 1
$$
which must be visited by $\gP$ since $s_x, s'_x \in \gS_x$ and $\gS_x = \text{supp}(\eta_x)$ by assumption. 

Consider $(f(s_x), g^{-1}(a_x), f(P_x(s_x, a_x)))$ and $(f(s'_x), g^{-1}(a_x), f(P_x(s'_x, a_x)))$. Both are visited by $\gP$, and have non-zero probability in $\hat{\rho}_{\hat{\pi}_x}^{P_x}({s}, {a}, {s}')$ the process in $\pi_x, P_x$ is positive recurrent (from the assumption that Markov chains by optimal policies are ergodic).


If ($D$) is true, then both triplets also have non-zero distribution in the stationary distribution of the process $\gQ$, i.e. we must have 
\begin{gather}
    (f(s_x), g^{-1}(a_x), f(P_x(s_x, a_x))) \in \text{supp}(\rho_{\pi_y}^{P_y}) \\
    (f(s'_x), g^{-1}(a_x), f(P_x(s'_x, a_x))) \in \text{supp}(\rho_{\pi_y}^{P_y})
\end{gather}
% as the pairs are both visited by $\gP$. and have non-zero probability in ${\rho}_{\pi_y}^{P, f, g}({s}, {a}, {s}')$ due to the process in $s_x$ being positive recurrent. 

However, due to the dynamics being deterministic in $\gM_y$, we must then have $$f(P_x(s_x, a_x)) = f(P_x(s_x', a_x)),$$ creating a contradiction, so ($D$) must be false.


% , O_y(f(s'_x), g^{-1}(a_x)) = 1, O_x(s_x, a_x) = 1, O_x(s'_x, a_x) = 1$, $f(s_x) = f(s_x')$ and $f(P_x(s_x, a_x)) \neq f(P_x(s_x', a_x))$. 

% yet optimal policy is preserved ($A$) and $\pi_x$ is an optimal policy in $\gM_x$. If $\lnot B$, then there exists $s_x, s'_x \in \gS_x$ and $a_x \in \gA_x$ such that $O_x(s_x, a_x) = 1, O_x(s'_x, a_x) = 1$, $f(s_x) = f(s_x')$ and $f(P_x(s_x, a_x)) \neq f(P_x(s_x', a_x))$ ($C$). 
% If ($D$) is true, then $(f(s_x), g^{-1}(a_x), f(P_x(s_x, a_x))) \in \text{supp}(\rho_{\pi_y}^{P_y})$ and $(f(s'_x), g^{-1}(a_x), f(P_x(s'_x, a_x))) \in \text{supp}(\rho_{\pi_y}^{P_y})$, as the pairs are optimal and are visited by $\pi_y$ and $P_y$. 

Combining the above four statements, we have $A \land B \iff C \land D$.
% If $(f, g^{-1}) \notin \gG(\gM_x, \gM_y)$ yet satisfies optimal policy preservation, then the dynamics preservation is violated, i.e. there exists $s_x$ and $s'_x$ such that $f(s_x) = f(s_x')$ yet for some optimal action $a_x$, $f(P_x(s_x, a_x)) \neq f(P_x(s_x', a_x))$. One of $(f(s_x), g^{-1}(a_x), f(P_x(s_x, a_x)))$ and $(f(s'_x), g^{-1}(a_x), f(P_x(s'_x, a_x)))$ must not appear in $\rho_{\pi_y}^{P_y}$ due to deterministic dynamics in $\gM_y$, yet appears in $\bar{\rho}_{\pi_x}^{P_x, f, g^{-1}}$. Therefore, $\rho_{\pi_y}^{P_y} = \bar{\rho}_{\pi_x}^{P_x, f, g^{-1}}$ must be violated, and we have verified the dynamics preservation property by contradiction.
% $\pi_y$ under two transition dynamics $P_y$ and $P_y^{f, g^{-1}}$. According to Lemma 2, $P_y = P_y^{f, g^{-1}}$ for all $(s_y, a_y, s'_y) \in \rho_{\pi_y}^{P_y}$ (otherwise $\rho_{\pi_y}^{P_y} \neq \rho_{\pi_y}^{P_y^{f, g^{-1}}}$, which violates the assumption). This verifies the transition dynamics preservation property.
\end{proof}





% \begin{align}
% f(P_{x}(s_{x}^{(t)}, g(\pi^{\circ}(s_{}  
% \end{align}
\begin{comment}
 Assume that at time $t$ some state $s_y \in \gS_y$ is supported under both $s_y^{(t)}$ and $\hat{s}_y^{(t)}$. The procedure that converges to $\sigma_{\pi_y}^{P_y}(s_y, a_y, s'_y)$ directly produces the next state distribution by $P_y(s_y, a_y)$, therefore $\Pr(s_y^{(t+1)} | s_y^{(t)})$ defines a transition kernel, and $s_y^{(t+1)}$ is independent from $\{s_y^{(i)}\}_{i=0}^{t-1}$ conditioned on $s_y^{(t)}$. 
The procedure that $\sigma_{\hat{\pi}_x}({s}_y, {a}_y, {s}'_y)$ indirectly produces the next state distribution by $f(P_x(s_x, g(a_y)))$ for some $s_x \in f^{-1}(s_y)$. The following equality shows that the conditional distribution of $s_y^{(t+1)}$ is also independent from $\{s_y^{(i)}\}_{i=0}^{t-1}$ conditioned on $s_y^{(t)}$, and is equal to the kernel define via $\pi_y$ and $P_y$.
\end{comment}



\begin{comment}
The goal is to first learn alignment maps on this task set then leverage the learned maps for CDIL, but a meaningful alignment may not always exist between every MDP pair. Intuitively, the MDPs must induce behaviors that have common structure \cite{Gupta2017Learning}. \todo{This statement needs to be revised depending the final state of the theory} In the following sections we formalize a notion of alignable MDPs for which a specific class of state, action maps that have provable transfer guarantees exist under suitable assumptions.
\end{comment}

\begin{comment}
In this work we assume access to an alignment task set $\mc{D}_{x, y} = \{(\mx_{, \T_{i}}, \my_{, \T_{i}})\}_{i = 1}^{N}$ where each MDP pair represents the same task $\T_{i}$ in the self and expert domains. The goal is to first learn alignment maps. A meaningful alignment may not always exist between every MDP pair. Intuitively, the MDPs must induce behaviors that have common structure \cite{Gupta2017Learning}. \todo{This statement needs to be revised depending the final state of the theory} In the following sections we formalize a notion of alignable MDPs for which a specific class of state, action maps that have provable transfer guarantees exist under suitable assumptions.


The goal is to first learn alignment maps $f: \sx \rightarrow \sy, g: \ay \rightarrow \ax$ such that the composite policy $\pi_{x, \T_{i}} = g \circ \pi^*_{y, \T_{i}} \circ f$ is optimal $\forall i$. The composite policy (Figure \ref{fig:setup}(b)) executes the following decision making process: given a state, imagine the related cross domain state, simulate the action that the expert would've taken from the imagined state, and finally pick the learner action that corresponds most closely to the simulated action. Then, given expert demonstrations $\{\tau^{(k)}_{y, \T_{new}}\}_{k = 1}^{K} \sim \pi^*_{y, \T_{new}}$ of a new task $\T_{new}$, we fit a expert policy model $\hat{\pi}^*_{y, \T_{new}}$ which can be composed with the alignment maps to construct a learner policy $\pi^*_{x, \T_{new}} = g \circ \hat{\pi}^*_{y, \T_{new}} \circ f$. Analogously, an infant that has already learned an association between his self state representation and an adult's physical state representation, should be able to rapidly imitate the adult demonstrating a new skill without much trial and error. 
\end{comment}






\begin{comment}
For succinctness of derivations we consider MDPs with discrete state, actions spaces and deterministic transition dynamics.

\subsection{Generative Adversarial Imitation Learning}
\js{paraphrase and we need to accurately introduce our setup.}
Suppose we do not have access to the ground truth reward signal $r$, but have demonstrations $\gD$ provided by an expert ($N$ expert agents in Markov games). The demonstrations $\gD$ is a set of trajectories $\{\tau_j\}_{j=1}^{M}$, where $\tau_j = \{(s^t_j, \va^t_j)\}_{t=1}^{T}$ is an expert trajectory collected by sampling $s^1 \sim \eta(s), \va^t \sim \pi_E(\va^t \vert s^t), s^{t+1} \sim P(s^{t+1} \vert s^t, \va^t)$.
$\gD$ contains the entire supervision to the learning algorithms, \emph{i.e.}, we cannot ask for additional interactions with the experts during training. Given $\gD$, imitation learning (IL) aims to directly learn policies that behave similarly to these demonstrations, whereas inverse reinforcement learning (IRL) \cite{russell1998learning, ng2000algorithms} seeks to infer the underlying reward functions which induce the expert policies.

In the context of imitation learning,~\citep{ho2016generative} proposed to use generative adversarial training \cite{goodfellow2014generative}, to learn the policies characterized by $\mathrm{RL} \circ \mathrm{IRL}(\pi_E)$ directly, leading to the Generative Adversarial Imitation Learning (GAIL) algorithm:
$$
\min_\theta \max_\omega \mathbb{E}_{\pi_E}\left[\log D_\omega(s,a)\right] + \mathbb{E}_{\pi_\theta}\left[\log(1 - D_\omega(s,a))\right]
$$
where $D_\omega$ is a discriminator that classifies expert and policy trajectories, and $\pi_\theta$ is the parameterized policy that tries to maximize its score under $D_\omega$. 
According to~\citet{goodfellow2014generative}, with infinite data and infinite computational capacities, at optimality, the distribution of generated state-action pairs should exactly match the distribution of demonstrated state-action pairs under the GAIL objective.
\end{comment}






\begin{comment}
In order to remove counfounding variables from our goal of assessing the efficacy of our alignment algorithm in uncovering reductions, we assume access to the full MDP simulator (which includes the reward function) for all MDP pairs in $D_{x, y}$, while on the test task we are only given samples of optimal behavior in the expert domain. 

Previous work in learning across morphologically different agents have assumed $(s^{(t)}_{x}, s^{(t)}_{y})$ are semantically correlated assuming that tasks are performed at the same rate (\cite{Gupta2017Learning}). The line of work revolving around manifold alignment \cite{Ammar2015Unsupervised} assumes the state space is a metric space and pairs states that have similar local topologies. The third person imitation learning approach aims to learn visual feature representations that maximally reduces domain information while preserving sufficient information about the state to choose an optimal action. 

Intuitively, we know that watching a robot staying still, doesn't teach us anything about running. 
(1). When will samples be useful?
(2). 

Humans are able to acquire new skills by observing morphologically different agents perform tasks. Ideally, AI agents should be equipped with such flexible imitation learning algorithms which are critical to the success active imitation learning in a world where virtually all agents have a unique morphology. We posit this cross domain knowledge extraction is an ability that emerges naturally once associations between internal self representations and physical state representations of other agents can be established. Analogously in humans, an infant's mind is constantly busy excavating similarities between himself and other agents in the world. (\todo{cite association paper}) We hypothesize that this association processes is strongly guided by functional similarity. Functionally similar states are both correlated with the attaining high performance on the similar tasks. Intuitively, infants are likely to associate their legs with those of an adult after observing that they are both used to perform the "walking" task. We argue that the ability to associate states across morphologically different agents based on functional similarity is a key ingredient to cross domain imitation learning. 

Visual similar states are close in the high-dimensional sensory input space while functionally similar states are strongly correlated with the attaining high performance on the similar tasks. As most visual observations are dynamic, a crucial property of visual stimuli is the temporal structure underlying it. Intuitively, infants are likely to associate their legs with those of an adult after observing that they are both used to perform the "walking" task, then find detailed associations between leg configurations that will generate similar temporal patterns in the generated sequence . 

We hypothesize that this learning process is guided by two evaluation metrics of similarity: visual and functional. Visual similarity is a comparison metric in the high-dimensional sensory input space while functional similarity is a metric in the abstracted feature space that only contains information relevant to performing a particular task. We argue that the ability to associate states across morphologically different agents based on functional similarity is a key ingredient to cross domain imitation. 
So we are given a dataset of paired MDPs that correspond to different agent's performing the same task. A mapping learned from each single task will pair up functionally similar states. 

Intuitively, body parts used by different agents to perform the same task should be closely associated and specific associations should be determined by matching temporal structure. 


Given a dataset of alignment tasks, learn a mapping such that $\pi_{x} = IL(f(\tau_{y}))$ is optimal.   

Functional similarity allows agents to learn associations in a feature space

Identifying similarities between agent's state representation and those of other agents is the key ingredient for imitation learning. 


In computer vision, finding functional similarities between images corresponds to learning representations that are useful for a particular task, whether it be classification, object detection, or segmentationis guided by label's which were determined by 

Consider an infant learning how to stack blocks by watching an adult perform the task. 

Consider a robot equipped with a library of primitive tasks where each skill is compactly represented as an MDP. An active learning robot should be able to acquire new skills by observing other agents perform tasks. In order to imitate a morphologically different agent, the robot first learns to associate his internal state representation with those of the other agent based two key components (1). visual similarity (2). functional similarity. Once 
\end{comment}



\begin{comment}
Let $\mc{D}_{x, y} = \{(\mx^{i}, \my^{i})\}_{i = 1}^{N}$ be a compatible alignment set comprising $N$ alignable MDP pairs for which there exists a shared reduction and $\pi_{y}^{i*}$ be the optimal expert policy for each pair. In order to remove counfounding variables from our goal of assessing the efficacy of our alignment algorithm in uncovering reductions, we assume access to the full MDP simulator (which includes the reward function) for all MDP pairs in $D_{x, y}$, while on the test task we are only given samples of optimal behavior in the expert domain. 
\end{comment}

\begin{comment}
\begin{align*}
& \Pr(\hat{s}_y^{(t+1)} = s'_y | \hat{s}_y^{(t)} = s_y) \\ 
& =   \int_{\ay} \int_{\sx} \Pr(s_x^{(t)} = s_x | \hat{s}_y^{(t)} = s_y) \Pr(\hat{a}_y^{(t)} = a_y | \hat{s}_y^{(t)} = s_y) \Pr(\hat{s}_y^{(t+1)} = s'_y | s_x^{(t)} = s_x, \hat{a}_y^{(t)} = a_y) \text{d} a_y \text{d} s_x \\
& = \int_{\ay} \int_{\sx}  \Pr(s_x^{(t)} = s_x | \hat{s}_y^{(t)} = s_y) \pi_y(a_y | s_y) \delta(s'_y = f(P_x(s_x, g(a_y))))\text{d} a_y  \text{d} s_x \\
& =  \int_{\ay} (\int_{\sx} \Pr(s_x^{(t)} = s_x | \hat{s}_y^{(t)} = s_y) \text{d} s_x) \pi_y(a_y | s_y) \delta(s'_y = P_y(s_y, a_y)) \text{d} a_y\\
& = \int_{\ay} \pi_y(a_y | s_y) \delta(s'_y = P_y(s_y, a_y))\text{d} a_y = \Pr(s_y^{(t+1)} = s'_y | s_y^{(t)} = s_y)
\end{align*}
\end{comment}




\begin{comment}
According to the assumptions over $\pi^{\circ}_y$ and the Markov chain defined via $\pi^{\circ}_y$ and $P_y$ being ergodic on $\gS_y$, we have
\begin{align*}
\forall s_y \in \gS_y, a_y \in \gA_y ~ \text{s.t} ~ O_y(s_y, a_y) = 1 &  \Rightarrow  \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T} \Pr(s_y^{(t)} = s_y; \pi^{\circ}_y, P_y) > 0 \\
&  \Rightarrow  \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T} \Pr(s_y^{(t)} = s_y; \pi_y, P_y) \pi^{\circ}_y(a_y | s_y) > 0 \\
& \Rightarrow  \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T} \Pr(s_y^{(t)} = s_y, a_y^{(t)} = a_y; \pi^{\circ}_y, P_y) > 0 \\
\end{align*}
i.e. $(s_y, a_y, P_y(s_y, a_y))$ is supported on $\sigyy(s_y, a_y, s'_y)$.

Because $\sigxy({s}_y, {a}_y, {s}'_y) = \sigyy(s_y, a_y, s'_y)$, we have $(s_y, a_y, P_y(s_y, a_y))$ is also supported on $\sigxy({s}_y, {a}_y, {s}'_y)$, i.e. running $\hat{\pi}_x$ would also visit the transition triple in $\gM_y$.For any state $s_x \in \gS_x$ consider its action $a_x \in \gA_x$ sampled from $\hat{\pi}_x(\cdot | s_x)$. From the definition of $\hat{\pi}_x$, $\exists a_y \in \gA_y$ such that $a_x = g(a_y)$. Because $\pi^{\circ}_{y}$ is an optimal mixture policy, $O_y(f(s_x), a_y) = 1$ if and only if $a_y \in \text{supp}(\pi^{\circ}_y(\cdot | f(s_x)))$. 

From the definition of $\hat{\pi}_x$ and the fact that $\hat{\pi}_x$ is optimal, we have $O_x(s_x, g(a_y)) = 1$ whenever $O_y(f(s_x), a_y) = 1$, which is equivalent to $O_y(\phi(s_x), \psi(g(a_y))) = 1$ since $\psi(g(a_y)) = a_y$. For all $a_x \in \gA_x$ such that $a_x \notin \Ima g$, we have set $\psi(a_x)$ such that $O_y(s_y, \psi(a_x)) = O_y(s_y, a_y^d) \neq 1$. Therefore, we have
\begin{align}
O_y(\phi(s_x), \psi(g(a_y))) = 1 \Rightarrow O_x(s_x, g(a_y)) = 1 \quad \forall s_{x} \in s_{x}, a_{x} \in \Ima g
\end{align}

\end{comment}


\begin{comment}
$\phi(s_{x}) = f(s_{x}), \psi(a_{x}) = g^{-1}(a_{x}), \forall s_{x} \in \text{supp}(\sigxx(s_{x})), a_{x} \in g(\ay)$ and $\phi(s_{x}) = s_{x}^{d}, \psi(a_{x}) = a_y^{d} ~~ \forall s_{x} \in \sx \setminus \text{supp}(\sigxx(s_{x})), a_{x} \in \ax \setminus g(\ay)$ where $a_{y}^{d}$ is a dummy action such that $O(s_{y}, a_{y}^{d}) = 0 ~~ \forall s_{y} \in \sy$. 
\end{comment}


\begin{comment}
We show the contrapositive, i.e $O_{\mx}(s_{x}, a_{x}) = 0 \Rightarrow O_{\my}(\psi(s_{x}), \psi(a_{x})) = 0 \quad \forall s_{x} \in \sx, a_{x} \in \ax$. Let $s_{x}^{-}, a_{x}^{-}$ be any suboptimal state action pair such that $O_{\mx}(s_{x}^{-}, a_{x}^{-})  = 0$. Since $\hat{\pi}_{x}$ is optimal, $(s_{x}^{-}, a_{x}^{-}) \notin \text{supp}(\sigxx(s_{x}, a_{x}))$. $\therefore O_{\my}(\psi(s_{x}^{-}), \psi(a_{x}^{-})) = 0$, concluding the proof. 
\end{comment}


\begin{comment}
In the following theorem, we show that given two MDPs, if we can find solutions that perfectly satisfy the objective, then the solutions are reductions, and thus the two MDPs are alignable. This shows that the satisfiability of the training objective is a sufficient test to whether two MDPs are alignable.

\begin{theorem}
\label{thm:main2}
Consider two unichain MDPs $\gM_x$ and $\gM_y$. Let $f: \gS_x \to \gS_y$ and $g: \gA_y \to \gA_x$ be two deterministic mappings, and let $\pi_x = g \circ \pi_y^{\circ} \circ f$ where $\pi_y^{\circ}$ is the optimal mixture policy for $\gM_y$, and assume $\text{supp}(\eta_x) = \gS_x$. % over $\gM_y$ such that $\forall s_y \in \gS_y, a_y \in \gA_y$, $O_y(s_y, a_y) = 1 \iff a_y \in \mathrm{supp}(\pi_y(\cdot | s_y))$. 
If there exists $f$ and $g$ such that (1). $g$ is injective, (2). $\pi_x \in \Pi^{*}_{\gM_x}$ and (3). $\sigxy({s}_y, {a}_y, {s}'_y) = \sigyy(s_y, a_y, s'_y)$ for all $s_y, s'_y \in \gS_y, a_y \in \gA_y$, then $\gM_y \leq \gM_x$ and $\exists (\phi, \psi) \in \Gamma(\gM_x, \gM_y)$ such that $\phi = f$ and $\psi \circ g(a_y) = a_y$ for all $a_y \in \gA_y$.
\end{theorem}

Intuitively, the two theorems tells us that if two MDPs are alignable, there exists a map that optimally achieves our training objective; conversely, if a map optimizes our training objective, it must be a reduction map between the two MDPs. Combined they imply that our training objective, if we can globally optimize it, finds a MDP reduction and the reduction "translates" the optimal expert policy $\pi_{y}$ into an optimal self policy $\pi_{x}$. 
\end{comment}


\begin{comment}
Since $(\phi, \psi)$ is a reduction, property (1) guarantees that $O_{\my}(\phi(s_{x}), \psi(\pi_{x}(s_{x}))) = 1 ~ \forall s_{x} \in \sx \Rightarrow O_{x}(s_{x}, \pi(s_{x})) = 1 ~ \forall s_{x} \in \sx$. We first see that 
\begin{align}
O_{\my}(\phi(s_{x}), \psi(\pi_{x}(s_{x}))) = O_{\my}(\phi(s_{x}), \psi(g(\pi_{y}(\phi(s_{x}))))) = O_{\my}(\phi(s_{x}), \pi_{y}(\phi(s_{x}))) = 1 ~~ \forall s_{x} \in \sx
\end{align}
where the first step substitutes the definition of $\pi_{x}$, the second step uses $\psi \circ g(a_{y}) = a_{y}$, and the last step follows from Corollary \ref{cor:optind}. Therefore, $O_{x}(s_{x}, \pi(s_{x})) = 1 ~ \forall s_{x} \in \sx$ which implies that $\pi_{x}$ is optimal by Lemma \ref{lemma:mixturepi}. The argument made above can be applied to stochastic policies by letting $\pi_{x}(s_{x})$ be a sample 
\end{comment}


\begin{comment}
\begin{proof}
$\forall s_x \in \sx, a_y \in \ay$, optimality of $\pi_y$ guarantees that:  
\begin{align}
    O_y(f(s_x), a_y) = 1 \iff a_y \in \text{supp}(\pi_y(\cdot | f(s_x)))
\end{align}
From the definition for policy $\hat{\pi}_x$, $\forall a_x \in \gA_x$, $a_x \in \text{supp}(\hat{\pi}_x(\cdot | f(s_x)))$ if and only if $\exists a_y \in \text{supp}(\pi_y(\cdot | f(s_x)))$ such that $a_x = g(a_y)$. Because of optimal policy preservation of $(\phi, \psi)$,
$$
O_y(\phi(s_x), \psi(a_x)) = 1 \Rightarrow O_x(s_x, a_x) = 1, \quad \forall s_x \in \gS_x, a_x \in \gA_x
$$
Substitute $a_x$ with $g(a_y)$:
\begin{align}
O_y(\phi(s_x), \psi(g(a_y))) = 1 \Rightarrow O_x(s_x, g(a_y)) = 1
\end{align}
Since $\psi(g(a_y)) = a_y$, $\phi = f$:
\begin{align}
O_y(f(s_x), a_y) = 1 \Rightarrow O_x(s_x, g(a_y)) = 1
\end{align}
Therefore 
\begin{align}
    a_y \in \text{supp}(\pi_y(\cdot | f(s_x))) \Rightarrow O_x(s_x, g(a_y)) = 1
\end{align}
which proves that all actions selected by $\hat{\pi}_x$ are optimal.
\end{proof}
\end{comment}


\begin{comment}
\begin{corollary}
\label{lemma:stationary-to-limiting}
For a unichain MDP $\mx$ with policy $\pi_{x}$ and transition dynamics $\px$, the triplet stationary distribution $\rho_{\pi_{x}}^{x}$ over $\sx \times \ax \times \sx$ is equal to the limiting mean distribution, defined as follows:
\begin{align}
    \sigxx(s_x, a_x, s'_x) = \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T-1} \Pr(s^{(t)}_x = s_x, a^{(t)}_x = a_x, s^{(t+1)}_x = s'_x)
\end{align}
\end{corollary}
\begin{proof}
This immediately follows from Lemmas~\ref{lemma:unichain-stationry} and~\ref{lemma:limit-mean}.
\end{proof}
\end{comment}


\begin{comment}
\begin{align*}
\sigxx(s_{x}, a_{x}) &=
  \begin{cases}
       \frac{\sigxx(s_{x}, a_{x}, s_{x}')}{\delta(s_{x}' - \px(s_{x}, a_{x}))} & \text{if $\delta(s_{x}' - \px(s_{x}, a_{x})) \neq 0$} \\
       0 & \text{otherwise} 
  \end{cases}
\\
\sigxx(s_{x}) &=
  \begin{cases}
       \frac{\sigxx(s_{x}, a_{x}, s_{x}')}{\delta(s_{x}' - \px(s_{x}, a_{x})) \hat{\pi}_{x}(a_{x} | s_{x})} & \text{if $\delta(s_{x}' - \px(s_{x}, a_{x})) \hat{\pi}_{x}(a_{x} | s_{x}) \neq 0$} \\
       0 & \text{otherwise} 
  \end{cases}
\end{align*}
\end{comment}

\begin{comment}
$\bullet$ Objective 1. $g$ is injective: assume that $\exists a_y, a'_y \in \gA_y$ such that $a_y \neq a'_y$ and $g(a_y) = g(a'_y)$. Then $a_y = \psi \circ g(a_y) = \psi \circ g(a'_y) = a'_y$, which contradicts our assumption that $a_y \neq a'_y$. 
\end{comment}


\begin{comment}
\begin{align}
\Pr(\hat{s}_y^{(t+1)} = s'_y | \hat{s}_y^{(t)} = s_y, \hat{a}_{y}^{(t)} = a_{y}; \mc{P}, \hat{\pi}_{x}) 
&= \delta(f(\px(s_{x}, g(a_{y}))) - s_{y}') ~~ \forall s_{x} \in f^{-1}(s_{y}) \label{eq:dy1}\\
&= \delta(\py(s_{y}, a_{y}) - s_{y}') \label{eq:dy2}\\
&= \Pr(s_y^{(t+1)} = s'_y | s_y^{(t)} = s_y, a_{y}^{(t)} = a_{y}; \py, \pi_{y})\\
\Pr(\hat{a}_{y}^{(t)} = a_{y} | \hat{s}_y^{(t)} = s_y) &= \pi_y(a_{y} | s_{y}) = \Pr(a_{y}^{(t)} = a_{y} | s_y^{(t)} = s_y)
\end{align}
\end{comment}

==> sections/related.tex <==
\section{Related Work}

Imitation learning (IL) approaches that address learning in the absence of an interactive oracle has revolved around behavioral cloning \cite{pomerleau1991efficient} and distribution matching \cite{ho2016generative, song2018multi}. In the conventional IL setting, demonstrations are assumed to be sampled from an expert domain equivalent to the self domain. To our knowledge, no previous work has formalized the cross domain imitation learning problem in which demonstrations are sampled from a (potentially) distinct MDP. 

Within the field of reinforcement learning (RL), transfer learning \cite{Taylor2009TransferSurvey}  between MDPs with identical state action spaces but different dynamics, has been explored in Atari games \cite{Rusu2016Progressive, Gamrian2018ImagetoImage} and sim-to-real transfer in robotics \cite{Tan2016SimtoReal}. A closely related field of cross domain transfer learning in the context of RL has explored approaches to find inter-state maps to exploit cross domain trajectories in a pretraining procedure that hopes to accelerate learning on a new task for which the reward function is available. Early works have hand-designed state maps \cite{Ammar2011SubspaceRL} or value function mappings \cite{taylor2007cross}. Canonical Correlation Analysis (CCA) \cite{Hotelling1936CCA} finds invertible projections into a basis in which the data from different domains are maximally correlated. These projections can then be composed to obtain a direct correspondence map between states. More recent works \cite{Ammar2015Unsupervised, Joshi2018Target} have utilized an unsupervised manifold alignment (UMA) algorithm which assumes the existence of hand crafted features along with a distance metric between them, then finds a linear map between states with similar local geometric properties. Instead of learning direct state maps, [1] assumes meaningful state pairings can be found via time alignment and instead focus on learning a domain invariant feature space. In contrast to this family of prior work, our approach exploits the latent structure of behaviors to learn both state, action maps in an unsupervised manner and considers the setting where reward function on the transfer task is unavailable. While we evaluate the usefulness of our learned MDP alignment maps as pretrained weights for comparison to prior work, we fundamentally desire to learn an optimal policy solely from cross domain demonstrations. 

Related to our proposed notion of MDP reductions, MDP homomorphisms \cite{Ranvindran2002Homo} have been explored with the aim of compressing state, action spaces to facilitate planning. With similar goals in mind, related works have proposed MDP similarity metrics based on bisimulation methods \cite{Ferns2004Bisumulation} and boltmzman machine reconstruction error \cite{Ammar2014Automated}. While conceptually related, these works have not proposed scalable procedures to discover the homomorphisms and have not drawn connections to cross domain learning. 


\begin{comment}
- General imitation learning: \\
Behavioral cloning \cite{pomerleau1991efficient} \\
GAIL \cite{ho2016generative} \\

- General Transfer learning in RL \\
General Survey \cite{Taylor2009TransferSurvey} \\
Progressive neural networks \cite{Rusu2016Progressive} \\
Image-to-Image translation for RL transfer \cite{Gamrian2018ImagetoImage}\\

- MDP homomorphism \\
barto \cite{Ranvindran2002Homo} \\
bisumlation methods \cite{Ferns2004Bisumulation} \\
automated mdp similarity (boltzman machine reconstruction) \cite{Ammar2014Automated}

- Cross domain transfer in RL \\
UMA \cite{Ammar2015Unsupervised} \\
CCA \cite{Hotelling1936CCA} \\
Cross domain transfer reinforcement learning (Peter Stone, others) \cite{taylor2007cross} \\
Target Apprentice \cite{Joshi2018Target}\\

- Learning across different morphology \\
invariant features \cite{Gupta2017Learning} \\
modular RL \cite{Devin2017Modular} \\

- Third person Learning \\
third person IL (original paper) \cite{stadie2017third} \\

- Domain adaptation and representation learning\\
MAML \cite{finn2017model} \\
CycleGAN \cite{zhu2017unpaired} \\
\end{comment}



==> sections/test.tex <==

\section{New}

An MDP is a tuple $(S,A,T,r,\rho)$.



\begin{definition}
Let $\mathcal{M}_x = (S_x,A_x,T_x,r_x,\rho_x)$ and $\mathcal{M}_y= (S_y,A_y,T_y,r_y,\rho_y)$ be two MDPs. Let $\left(s_x^{(0)}, \cdots,s_x^{(N)}\right)$ the stochastic process representing the sequence of states under optimal policy $\pi^*_x$ and initial state distribution $\rho_x$. 
Let $\left(s_y^{(0)}, \cdots,s_y^{(N)}\right)$ the sequence of states under optimal policy $\pi^*_y$ and initial state distribution $\rho_y$.


A (surjective?) mapping $f:S_x \rightarrow S_y$ 
is a reduction if
for all $N\geq 0$
$\left(f(s_x^{(0)}), \cdots, f(s_x^{(N)})\right)$ and $\left(s_y^{(0)}, \cdots,s_y^{(N)}\right)$ are identically distributed.
We say $\mathcal{M}_x \succ \mathcal{M}_y$ if a reduction exists.
\end{definition}

Define
$$
\rho_{\pi_x}^{N}(s, a, s') = \frac{1}{N} \sum_{t=0}^{N} P (s_x^{(t)} = s, a_x^{(t)} = a, s_x^{(t+1)}=s')
$$

\begin{theorem}
\label{thm:main}
If $\mathcal{M}_x \succ \mathcal{M}_y$, and $\pi_y$ is an optimal policy over $\mathcal{M}_y$. Let $f: \gS_x \to \gS_y$ and $g: \gA_y \to \gA_x$ be two deterministic mappings, and $\pi_x = g \circ \pi_x \circ f$. Specifically, $\pi_x$ selects an action $a_x$ given a certain state $s_x$ by mapping it to $f(s_x)$, obtaining an action $a_y$ from $\pi_y(\cdot|f(s_x))$ and the obtaining its action $a_x = g(a_y)$.

Then
$$
\pi_x \text{ is optimal in } \gM_x \text{ and } \forall N, \rho_{\pi_y}^{N} = \rho_{\pi_x}^{N} \Rightarrow \textrm{$f$ is a reduction}
$$
\end{theorem}


==> sections/transfer.tex <==
\section{Transfer learning analysis}
Now that we specified an approach to discover a shared structure (homomorphism) between two MDPs, we are interested in more general cases involving sets of MDPs. Let $\gD_x = \{\gM_x^i\}_{i=1}^N$ and $\gD_y = \{\gM_y^i\}_{i=1}^N$ denote two sets of MDPs in domains $x$ and $y$ containing $N$ elements each; we assume that all the elements in $\gD_x$ have the same state space, action space, transition dynamics and only differ in terms of the reward function; the same goes for $\gD_y$. We are interested of finding alignments over the set of MDP pairs $\gD = \{(\gM_x^i, \gM_y^i)\}_{i=1}^N$ which is also an alignment over some unknown test MDP pair $(\gM_x^T, \gM_y^T)$. We define $\Gamma(\gD) = \cap_{i \in [N]} \Gamma(\gM_x^i, \gM_y^i)$ be the valid alignments over all the pairs of MDPs in $\gD$.

\begin{definition}
$\gD$ is transferable to $(\gM_x^T, \gM_y^T)$ if $\Gamma(\gD) \subseteq \Gamma(\gM_x^T, \gM_y^T)$.
\end{definition}

If $\gD$ is transferable to $(\gM_x^T, \gM_y^T)$, then any alignment we found for $\gD$ is also an alignment valid for $(\gM_x^T, \gM_y^T)$, which would allow us to perform zero-shot transfer from the optimal policy in $\gM_y$ to an optimal policy in $\gM_x$.

\begin{theorem}
Assume $b(\cdot): \{0, 1\}^N \to \{0, 1\}$ is some boolean expression over $\{0, 1\}^N$ that can be written as a canonical disjunctive normal form (CDNF) where all of the minterms does not contain nots, i.e. $b(c_1, \ldots, c_N) = \sum_C \prod_{c_i \in C} c_i$ where $C \subseteq \{c_1, \ldots, c_N\}$. If $O_{\gM_y^T}(s_y, a_y) = b(\{O_{\gM_y^i}(s_y, a_y)\}_{i=1}^{N})$ and $O_{\gM_x^T}(s_x, a_x) = b(\{O_{\gM_x^i}(s_x, a_x)\}_{i=1}^{N})$, then $\gD$ is transferable to $(\gM_x^T, \gM_y^T)$.
\end{theorem}
\begin{proof}
We show that $(\phi, \psi) \in \Gamma(\gM_x^T, \gM_y^T)$ for all $(\phi, \psi) \in \Gamma(\gD)$. 
First, we verify that the conditions for optimal policy preservation holds, i.e. 
$$
O_{\gM_y^T}(\phi(s_x), \psi(a_x)) = 1 \Rightarrow O_{\gM_x^T}(s_x, a_x) = 1, \quad \forall s_x \in \gS_x, a_x \in \gA_x
$$ 
If $O_{\gM_y^T}(\phi(s_x), \psi(a_x)) = 1$, then in its CDNF form, at least one of the minterms is true; without loss of generalization, we denote one of the minterms evaluated as true as $$\prod_{i \in \gI} O_{\gM_y^i}(\phi(s_x), \psi(a_x))$$ where $\gI \in \{1, \ldots, N\}$ denotes an index set. Therefore $O_{\gM_y^i} \land O_y^{j} = 1$ for all $i \in \gI$. Because $(\phi, \psi) \in \Gamma(\gD)$ optimal policy preservation holds for all pairs in $\gD$, so for all $i \in \gI$, $O_{\gM_x^i}(s_x, a_x) = 1$; thus, $O_{\gM_x^T}(s_x, a_x) = b(\{O_{\gM_x^i}(s_x, a_x)\}_{i=1}^{N}) = 1$ and the optimal policy preservation holds. 

Next, because dynamics preservation holds for all $(\gM_x^i, \gM_y^i)$ pairs, we have for all $i \in [N]$:
$$
\py^i(s_{y}, a_{y}) = \phi^i(\px(s_{x}, a_{x})) \quad \forall s_{x} \in \phi^{-1}(s_{y}), a_{x} \in \psi^{-1}(a_{y})
$$
for all $s_y \in \gS_y, a_y \in \gA_y$ where $O_{\my}^i(s_{y}, a_{y}) = 1$ holds. Therefore, for all $s_y \in \gS_y, a_y \in \gA_y$, either $O_{\my}^T(s_{y}, a_{y}) = 0$, or $O_{\my}^T(s_{y}, a_{y}) = 1$, which indicates $\exists i \in [N]$ such that $O_{\my}^i(s_{y}, a_{y}) = 1$. 

Thus we have 
$$
\py^i(s_{y}, a_{y}) = \phi^i(\px(s_{x}, a_{x})) \quad \forall s_{x} \in \phi^{-1}(s_{y}), a_{x} \in \psi^{-1}(a_{y})
$$
for all $s_y \in \gS_y, a_y \in \gA_y$ where $O_{\my}^T(s_{y}, a_{y}) = 1$ holds, and from such, $(\phi, \psi)$ should also satisfy the dynamics preservation over $(\gM_x^T, \gM_y^T)$.
\end{proof}
